FLAME: Frozen Large Language Models Enable Data-Efficient Language-Image Pre-training

Language-image pre-training faces significant challenges due to limited data in specific formats and the constrained capacities of text encoders. While prevailing methods attempt to address these issues through data augmentation and architecture modifications, they continue to struggle with processing long-form text inputs, and the inherent limitations of traditional CLIP text encoders lead to suboptimal downstream generalization. In this paper, we propose FLAME (Frozen Large lAnguage Models Enable data-efficient language-image pre-training) that leverages frozen large language models as text encoders, naturally processing long text inputs and demonstrating impressive multilingual generalization. FLAME comprises two key components: 1) a multifaceted prompt distillation technique for extracting diverse semantic representations from long captions, which better aligns with the multifaceted nature of images, and 2) a facet-decoupled attention mechanism, complemented by an offline embedding strategy, to ensure efficient computation. Extensive empirical evaluations demonstrate FLAME's superior performance. When trained on CC3M, FLAME surpasses the previous state-of-the-art by 4.9% in ImageNet top-1 accuracy. On YFCC15M, FLAME surpasses the WIT-400M-trained CLIP by 44.4\% in average image-to-text recall@1 across 36 languages, and by 34.6% in text-to-image recall@1 for long-context retrieval on Urban-1k. Code is available at https://github.com/MIV-XJTU/FLAME.

==> tables/dci_docci.tex <==
\begin{table}[t]
\small
\centering
\resizebox{\linewidth}{!}{
\begin{NiceTabular}{l|l|cc|cc}
% \toprule
& & \multicolumn{2}{c}{DCI} & \multicolumn{2}{c}{DOCCI-test} \\
Method & Dataset & I2T & T2I & I2T & T2I\\
\midrule[1pt]
CLIP~\cite{radford2021clip} & CC3M & 8.3 & 7.5 & 8.6 & 7.0 \\
Long-CLIP~\cite{zhang2024long-clip} & CC3M+S4V & 13.8 & 14.2 & 14.7 & 12.6 \\
FLAME & CC3M & \cellcolor{gray!10}\textbf{50.8} & \cellcolor{gray!10}\textbf{49.3} & \cellcolor{gray!10}\textbf{54.5} & \cellcolor{gray!10}\textbf{51.9} \\
\midrule
CLIP~\cite{radford2021clip} & YFCC15M & 22.0 & 19.1 & 26.5 & 23.3 \\
Long-CLIP~\cite{zhang2024long-clip} & YFCC15M+S4V & 29.4 & 29.7 & 35.0 & 33.5 \\
FLAME & YFCC15M & \cellcolor{gray!10}\textbf{66.1} & \cellcolor{gray!10}\textbf{68.1} & \cellcolor{gray!10}\textbf{75.8} & \cellcolor{gray!10}\textbf{76.2} \\
\midrule
CLIP~\cite{radford2021clip} & WIT-400M & 45.4 & 43.0 & 60.7 & 57.0 \\
\end{NiceTabular}
}
\vspace{-5pt}
\caption{\textbf{Long-context retrieval recall@1 results on DCI and DOCCI test set.} S4V denotes ShareGPT4V.}
\label{tab:dci_docci}
\vspace{-.5em}
\end{table}
